Implicit Mesh Reconstruction from Unannotated Image Collections

We present an approach to infer the 3D shape, texture, and camera pose for an object from a single RGB image, using only category-level image collections with foreground masks as supervision. We represent the shape as an image-conditioned implicit function that transforms the surface of a sphere to that of the predicted mesh, while additionally predicting the corresponding texture. To derive supervisory signal for learning, we enforce that: a) our predictions when rendered should explain the available image evidence, and b) the inferred 3D structure should be geometrically consistent with learned pixel to surface mappings. We empirically show that our approach improves over prior work that leverages similar supervision, and in fact performs competitively to methods that use stronger supervision. Finally, as our method enables learning with limited supervision, we qualitatively demonstrate its applicability over a set of about 30 object categories.

==> impact.tex <==
\section*{Broader Impact}
The long term goal of our research direction is to build robust perception systems that perceive accurate spatial structure of objects and scenes. Eventually, we envision a world where 3D perception is ubiquitous -- that 3D inference from images would be a basic technology accessible to everyone \eg an interior designer should be able to recover and modify the structure of a room from an image, a game designer should be able to import objects from the real world into the virtual one, a robotics researcher should feel assured that their agent will `see' that the plate is flat. Just as our advances in 2D recognition have revolutionized various aspects of our lives \eg photography, shopping \etc, we expect `success' at 3D understanding to be similarly transformative. While there are effects we can anticipate \eg impact in graphics, content creation, virtual and augmented reality, there will also of course be possible unanticipated (and possibly undesirable) consequences. In addition to the vision and graphics applications though, the ability to infer the spatial structure of the world is a basic capability we humans possess, and one that we argue any autonomous agent critically requires.We therefore hope our research also takes us a step closer to building autonomous agents that perceive and interact with the world.

==> pck_r.tex <==
\begin{table}[h]
\tablelabel{pcktransfer}
\setlength{\tabcolsep}{8pt} 
\centering 
% \small{
\scalebox{1.0}{
\begin{tabular}{@{}ll|rrrrr@{}} \toprule
% \multicolumn{2}{c}{Item} \\ \cmidrule(r){1-2}
Supv & Method & Birds & Horses   & Cows &Sheep\\ \midrule
\multirow{2}{1cm}{KP + Mask}
 & CMR  & 80.0 &  &  &  \\
 & Rigid-CSM  & 68.5 & 46.4 & 52.6 & 47.9 \\
 & A-CSM & 72.4 & 57.3 & 56.8 & 57.4 \\
 & IMR & 90.8 & 63.4 & 62.0 & 59.4 \\
\midrule
\multirow{2}{1cm}{Mask} & Rigid-CSM & 50.9 & 49.7 & 37.4 & 36.4 \\
  &   A-CSM & 46.8 & 54.2 & 43.8 & 42.5 \\
  &   IMR (fixed $\bar{\phi}$) & 53.9 & 51.0 & 46.9 & 45.5 \\
  &   IMR (contour, fixed $\bar{\phi}$) & 51.4 & 55.4 & 52.9 & 45.0 \\
% &   IMR (contour, fixed $\bar{\phi}$, normal loss) & 59.9 & 48.0 & 43.9 & 41.7 \\
&   IMR (contour, fixed $\bar{\phi}$) - GCC & 49.5 & 55.1  & 39.8  & 41.0 \\\bottomrule
\end{tabular}
}
\vspace{2mm}
\caption{{\bf Keypoint Reprojection Accuracy} 
% The best numbers are in \textbf{bold}.
}
\end{table}


\begin{table}[h]
\tablelabel{pcktransfer}
\setlength{\tabcolsep}{8pt} 
\centering 
% \small{
\scalebox{1.0}{
\begin{tabular}{@{}ll|rrrrrr@{}} \toprule
% \multicolumn{2}{c}{Item} \\ \cmidrule(r){1-2}
Metric & Method & Birds & Horses  & Cows & Sheep & Car \\
\midrule
\multirow{2}{1.2cm}{PCK-R}
  &  S2 & 52.5  & 46.2  & 33.2  & 32.4  & 38.2  \\
  &  S2 + edge & 53.1  & 46.7  & 35.0  & 32.7  & 38.5 \\
  &  S2 + dt & 50.5 & 46.9  & 34.1  & 34.2  & 39.2  \\
    &  S2 + edge + dt &  53.2 & 46.9  & 36.4 & 35.3 & 38.6 \\
\midrule
\multirow{2}{1.2cm}{PCK-T}
  &  S2 & 54.2  & 59.1 & 51.8 & 47.0 & 54.2 \\
  &  S2 + edge & 59.0  & 59.1  & 52.9 & 47.6 & 54.3 \\
  &  S2 + dt &  46.2 & 57.5 & 53.1 & 43.6 &  55.3 \\
    &  S2 + edge + dt & 50.1  & 59.2  & 53.3 & 48.7 & 55.2 \\
\bottomrule
\end{tabular}
}
\vspace{2mm}
\caption{{\bf Stage2 losses ablation.} All nets partially trained.
}
\end{table}


==> pck_t.tex <==
\begin{table}[h]
\tablelabel{pcktransfer}
\setlength{\tabcolsep}{8pt} 
\centering 
% \small{
% \scalebox{1.0}{
\begin{tabular}{@{}ll|rrrrr@{}} \toprule
% \multicolumn{2}{c}{Item} \\ \cmidrule(r){1-2}
Supv & Method & Birds & Horses   & Cows & Sheep & Car \\ \midrule
\multirow{2}{1cm}{KP + Mask}
 & CMR  & 47.3 &  &  &  \\
 & Rigid-CSM  & 45.8 & 42.1 & 28.5 & 31.5 \\
 & A-CSM  & 51.0   & 44.6 & 29.2 & 39.0 \\
% & R-CSM w. IT-fixed (ITF)  & 70.8  \\
% & R-CSM w. IT-learned  & 69.8    \\ 
% & R-CSM w. ITF+Def  & 69.9 \\
% & R-CSM w. ITF+Def+Sym  & 69.2 \\ 
% & R-CSM w. ITF [mc,sym (g+l)]  & 54.9 & 42.7  & 35.8  & 32.2  &  \\
% & R-CSM w. ITF  & 56.0 & 45.6 & 32.1  & 28.1  &  \\
%c& R-CSM w. ITL [mc,sym (g+l)]  & 60.0 & 44.9  & 37.3  & 34.2 &  \\
% & R-CSM w. ITL  & 60.8 & 46.6 & 32.3 & 33.4  &  \\
& IMR  & 63.8 & 47.3 & 37.4 & 36.9  &  \\
\midrule
\multirow{2}{1cm}{Mask} &  Dense-Equi & 33.5 & 23.3 & 20.9 & 19.6 & 31.5 \\
& Rigid-CSM & 36.4 & 31.2 & 26.3 & 24.7 & 40.0 \\
&  A-CSM  & 42.6 & 32.9 & 26.3 & 28.6 \\
& IMR  & 56.1  & 39.1 &  31.1 & 27.3 & 41.3 \\  
&   IMR (fixed $\bar{\phi}$) & 50.0 & 43.6 & 31.0 & 31.1 & 38.5 \\
& IMR (contour)  & 55.4  & 44.6 &  32.6 & 30.2 & 42.4 \\
&   IMR (contour, fixed $\bar{\phi}$) & 54.9 & 43.7  & 34.1 &  27.3 & 41.8 \\
% &   IMR (contour, fixed $\bar{\phi}$, normal loss) & 54.0 & 40.9 & 33.7 & 30.6  & 39.3  \\
&   IMR (contour, fixed $\bar{\phi}$) - GCC & 49.2 & 40.3 &  33.0 & 27.0  & 40.4  \\
\bottomrule
\end{tabular}
\vspace{2mm}
\caption{{\bf PCK-Transfer for Evaluating CSM Prediction}.}
% }

\end{table}



